R-STELLAR: A Resilient Synthesizable Signature Attenuation SCA Protection on AES-256 with built-in Attack-on-Countermeasure Detection

Side channel attacks (SCAs) remain a significant threat to the security of cryptographic systems in modern embedded devices. Even mathematically secure cryptographic algorithms, when implemented in hardware, inadvertently leak information through physical side channel signatures such as power consumption, electromagnetic (EM) radiation, light emissions, and acoustic emanations. Exploiting these side channels significantly reduces the search space of the attacker. In recent years, physical countermeasures have significantly increased the minimum traces to disclosure (MTD) to 1 billion. Among them, signature attenuation is the first method to achieve this mark. Signature attenuation often relies on analog techniques, and digital signature attenuation reduces MTD to 20 million, requiring additional methods for high resilience. We focus on improving the digital signature attenuation by an order of magnitude (MTD 200M). Additionally, we explore possible attacks against signature attenuation countermeasure. We introduce a Voltage drop Linear region Biasing (VLB) attack technique that reduces the MTD to over 2000 times less than the previous threshold. This is the first known attack against a physical side-channel attack (SCA) countermeasure. We have implemented an attack detector with a response time of 0.8 milliseconds to detect such attacks, limiting SCA leakage window to sub-ms, which is insufficient for a successful attack.

==> source_inputs/biographies.tex <==
\begin{comment}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ISCC JPG.jpg}}] {Archisman Ghosh} received the Bachelor of Electronics and Telecommunication Engineering degree from Jadavpur University, Kolkata, India, in 2017. He worked as Digital Design Verification Engineer at Samsung Semiconductor Institute R\&D (SSIR) before joining the Ph.D. degree in electrical and computer engineering at Purdue University, West Lafayette, IN, USA, working with Prof. Shreyas Sen. His research interests include mixed-signal IC design and hardware security.

During his Ph.D., he has been awarded the ECE Fellowship for academic excellence during 2019–2020.He has been serving as a primary reviewer for multiple reputed journal \& conferences including VLSID, Springer WPC.
 \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{debayan_das.png}}]{Debayan Das} (S'17) is a Ph.D. student in Electrical and Computer Engineering at Purdue University, working with Professor Shreyas Sen. He received his Bachelor of Electronics and Telecommunication Engineering from Jadavpur University, India, in 2015. Prior to joining PhD, he worked as an Analog Design Engineer at a start-up based in India. He has interned with the Security Research Lab, Intel Labs, OR, over the summers of 2018 and 2020. His research interests include mixed-signal IC design and hardware security.

Debayan was a recipient of the IEEE HOST Best Student Paper Award in 2017, 2019, and the 3rd Best Poster Award in IEEE HOST 2018. In 2019, one of his papers was recognized as a Top Pick in Hardware \& Embedded Security published over the span of last six years. He was recognized as the winner (third place) of the ACM ICCAD 2020 Student Research Competition (SRC). During his Ph.D., he has been awarded the ECE Fellowship during 2016–2018, the SSCS Pre-doctoral Achievement Award in 2020-21, and the Bilsland Dissertation Fellowship and the Best Graduate  during the final year (2020–2021) for his outstanding overall achievements.
\end{IEEEbiography}
\vspace{-5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{josef_danial.png}}]{Josef Danial} received his B.Sc. in Computer Engineering from Purdue University, West Lafayette, IN, USA, in 2018. He has two years of industry experience, in automotive (Fiat Chrysler Automobiles) and IOT (Cisco Jasper) companies. Now he is pursuing his Master's degree with the SPARC Lab, Purdue University as a Graduate Research Assistant. His research interests include machine learning, hardware security, and computer vision.
\end{IEEEbiography}
\vspace{-2cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{santosh ghosh bio.jpg}}]{Santosh Ghosh} is a Research Scientist in Intel Labs. He has coauthored about 65 research publications in refereed international conferences and journals with a citation H-index of 21, and 20 issued with other 51 more patents filed (pending). The primary focus of his research includes: 1) design and implement cryptographic hardware microarchitecture and RTL with the aggressive area, latency, and throughput constraints; multiple of them are already being deployed in high-volume Intel products; 2) investigate and develop timing, power, and EM side-channel countermeasures; and 3) collaborate with academic partners and provide cryptography and security guidance to Intel business units. Santosh received the Ph.D. degree from IIT Kharagpur, India in 2011, and completed his post-doctoral studies from COSIC, KU Leuven, Leuven, Belgium, in the area of cryptographic hardware and side-channel attacks.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Vivek de photo.JPG}}]
{Vivek De} is an Intel Fellow and Director of Circuit Technology Research in Intel Labs. He is responsible for providing strategic technical directions for long term research in future circuit technologies and leading energy efficiency research across the hardware stack. He has 327 publications in refereed international conferences and journals with a citation H-index of 83, and 236 patents issued with 27 more patents filed (pending). He received an Intel Achievement Award for his contributions to an integrated voltage regulator technology. He is the recipient of the 2019 IEEE Circuits and System Society (CASS) Charles A. Desoer Technical Achievement Award for “pioneering contributions to leading-edge performance and energy-efficient microprocessors \& many-core system-on-chip (SoC) designs” and the 2020 IEEE Solid-State Circuits Society (SSCS) Industry Impact Award for “seminal impact and distinctive contributions to the field of solid-state circuits and the integrated circuits industry”. He received a Best Paper Award at the 1996 IEEE International ASIC Conference, and nominations for Best Paper Awards at the 2007 IEEE\/ACM Design Automation Conference (DAC) and 2008 IEEE/ACM International Conference on Computer\-Aided Design (ICCAD). He also co-authored a paper nominated for the Best Student Paper Award at the 2017 IEEE International Electron Devices Meeting (IEDM). One of his publications was recognized in the 2013 IEEE/ACM Design Automation Conference (DAC) as one of the "Top 10 Cited Papers in 50 Years of DAC". Another one of his publications received the “Most Frequently Cited Paper Award” in the IEEE Symposium on VLSI Circuits at its 30th Anniversary in 2017. He was recognized as a Prolific Contributor to the IEEE International Solid-State Circuits Conference (ISSCC) at its 60th Anniversary in 2013, and a Top 10 Contributor to the IEEE Symposium on VLSI Circuits at its 30th Anniversary in 2017. He received the Outstanding Evening Session Award at the 2018 International Solid-State Circuits Conference (ISSCC). He served as an IEEE/EDS Distinguished Lecturer in 2011, an IEEE/SSCS Distinguished Lecturer in 2017-18, and an IEEE/CASS Distinguished Lecturer in 2020-22. He received the 2017 Distinguished Alumnus Award from the Indian Institute of Technology (IIT) Madras. He received a B.Tech from IIT Madras, India, a MS from Duke University, Durham, North Carolina, and a PhD from Rensselaer Polytechnic Institute, Troy, New York, all in Electrical Engineering. He is a Fellow of the IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{shreyas_sen.jpg}}]{Shreyas Sen} (S’06–M’11–SM’17) is an Associate Professor in ECE, Purdue University and received his Ph.D. degree in ECE, Georgia Tech. Dr. Sen has over 5 years of industry research experience in Intel Labs, Qualcomm and Rambus. His current research interests span mixed-signal circuits/systems and electromagnetics for the Internet of Things (IoT), Biomedical, and Security. Dr. Sen is the inventor of the Electro-Quasistatic Human Body Communication, for which, he is the recipient of the MIT Technology Review top-10 Indian Inventor Worldwide under 35 (MIT TR35 India) Award. Dr. Sen's work has been covered by 100+ news releases worldwide, invited appearance on TEDx Indianapolis, Indian National Television CNBC TV18 Young Turks Program and NPR subsidiary Lakeshore Public Radio. Dr. Sen is a recipient of the NSF CAREER Award 2020, AFOSR Young Investigator Award 2016, NSF CISE CRII Award 2017, Google Faculty Research Award 2017, Intel Labs Quality Award for industrywide impact on USB-C type, Intel Ph.D. Fellowship 2010, IEEE Microwave Fellowship 2008 and seven best paper awards including IEEE CICC 2019 and IEEE HOST 2017, 2018, and 2019. Dr. Sen's work was chosen as one of the top-10 papers in the Hardware Security field over the past 6 years (TopPicks 2019). He has co-authored 2 book chapters, over 135 journal and conference papers, and has 14 patents granted/pending. He serves/has served as an Associate Editor for IEEE Design \& Test, Executive Committee member of IEEE Central Indiana Section and Technical Program Committee member of DAC, CICC, DATE, ISLPED, ICCAD, ITC, VLSI Design, among others. Dr. Sen is a Senior Member of IEEE.
\end{IEEEbiography}

\end{comment}
